Few-Shot Semantic Parsing for New Predicates

In this work, we investigate the problems of semantic parsing in a few-shot learning setting. In this setting, we are provided with utterance-logical form pairs per new predicate. The state-of-the-art neural semantic parsers achieve less than 25% accuracy on benchmark datasets when k= 1. To tackle this problem, we proposed to i) apply a designated meta-learning method to train the model; ii) regularize attention scores with alignment statistics; iii) apply a smoothing technique in pre-training. As a result, our method consistently outperforms all the baselines in both one and two-shot settings.

==> ablation-result_back.tex <==
\begin{table*}[ht]
\small
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|@{} |l|ccc@{}||ccc@{}|}
\toprule
         & \Jobs & \Geo & \Atis  & \Jobs & \Geo & \Atis \\ 
\midrule
Ours  &27.09 \pm 4.14 & \textbf{27.49 $\pm$ 11.25}         & \textbf{19.27 $\pm$ 7.73}  & \textbf{32.50 $\pm$ 11.18} & \textbf{48.45 $\pm$ 5.71}       & \textbf{22.48 $\pm$ 3.82}   \\
\hline
\quad - sup  & 23.63 $\pm$ 7.19 & 18.86 $\pm$ 9.94  & 12.91 $\pm$ 3.75 & 26.91 $\pm$ 7.72 & 39.51 $\pm$ 9.23  & 14.89 $\pm$ 3.90 \\

\quad -  proto  & 22.91 $\pm$ 5.16 & 18.77 $\pm$ 9.99  & 13.24 $\pm$ 5.33 & 29.16 $\pm$ 4.92 & 38.93 $\pm$ 6.10  & 16.81 $\pm$ 4.86 \\
\hline
\quad -  reg  & \textbf{29.27 $\pm$ 5.16} & 18.10 $\pm$ 9.68 & 13.66 $\pm$ 4.46 & 31.03 $\pm$ 8.40 & 39.61 $\pm$ 7.02 & 18.58 $\pm$ 4.84 \\

\quad -  strsim  & 22.18 $\pm$ 8.62 & 19.62 $\pm$ 6.76 & 10.14 $\pm$
6.71 & 28.41 $\pm$ 8.38 & 47.09 $\pm$ 3.93 & 19.84 $\pm$
5.41 \\

\quad -  cond  & 23.27 $\pm$ 8.73 & 19.05 $\pm$ 6.74 & 9.50 $\pm$
5.77 & 27.66 $\pm$ 7.95 & 40.97 $\pm$ 3.25 & 17.50 $\pm$
5.82 \\
\hline
%\quad - idiom & 15.45 $\pm$ 4.68  & 22.75 $\pm$ 5.87        & 17.74 $\pm$ 10.40  & 19.25 $\pm$ 8.45  & 43.88 $\pm$ 10.12        & \textbf{22.77 $\pm$ 3.21}     \\

\quad - smooth  & 24.36 $\pm$ 4.33  & 23.60 $\pm$ 13.87        & 15.23 $\pm$ 10.45  & 30.84 $\pm$ 9.06  & 44.95 $\pm$ 6.15        & 18.71 $\pm$ 1.09     \\
%\hline
\bottomrule
\end{tabular}%
}
\caption{Ablation study results. (Left) The one-shot learning results. (Right) The two-shot learning results.}
\label{table:ablation}
\vspace{-2mm}
\end{table*}
%\begin{table}[ht]
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{@{} l|ccc@{}}
%\toprule
%         & \Jobs & \Geo & \Atis \\ 
%\midrule
%- sup & 26.91 $\pm$ 7.72 & 39.51 $\pm$ 9.23  & 14.89 $\pm$ 3.90  \\

%-  proto & 29.16 $\pm$ 4.92 & 38.93 $\pm$ 6.10  & 16.81 $\pm$ 4.86  \\
%\hline
%- reg & 31.03 $\pm$ 8.40 & 39.61 $\pm$ 7.02 & 18.58 $\pm$ 4.84 \\
%\hline
%- norm & 19.25 $\pm$ 8.45  & 43.88 $\pm$ 10.12        & \textbf{22.77 $\pm$ 3.21}    \\

%- smooth & 30.84 $\pm$ 9.06  & 44.95 $\pm$ 6.15        & 18.71 $\pm$ 1.09    \\
%\hline
%Ours & \textbf{32.50 $\pm$ 11.18} & \textbf{49.32 $\pm$ 3.18}       & 22.48 $\pm$ 3.82    \\
%\bottomrule
%\end{tabular}%
%}
%\caption{Ablation study results of two shot learning results}
%\label{table:ablation-two}
%\end{table}

==> alg-dropout_back.tex <==
\begin{algorithm}[t]
{\small
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\SetAlgoLined
\Input{Training set $\mathcal{D}$, a predicate set $\mathcal{P}$,     a supervised trained predicate embedding $\mathcal{C}_s$, number of shots $k$, number of queries $n$ per predicate}
\Output{The loss $\mathcal{L}_m$.}
    Sample a subset $\mathcal{P}_i \sim \mathcal{P}$\\ 
    $S$ := $\emptyset$\\ 
    $Q$ := $\emptyset$\\
    \For{p in $\mathcal{P}_i$}{
        Sample $S'$ of size $k$ from $\mathcal{D}_p$\\
        Sample $Q'$ of size $k$ $\times$ $n$ from $\mathcal{D}_p$\\
        $S = S \cup S'$\\
        $Q = Q \cup Q'$\\
    }
    Build a prototype matrix $\mathcal{C}_p$ on $S$\\
    Build a mask $\mathbf{m}$ using $\mathcal{P}_i$\\
    Apply Eq. \eqref{eq:action_embed_meta} to compute $\mathbf{C}'$\\
    Compute $\mathcal{L}_m$, the cross-entropy on $Q$ with $\mathbf{C}'$\\
%    Compute $\mathcal{L} = \mathcal{L}_s + \mathcal{L}_m$ + \lambda \Omega \\

}
\caption{Predicate-Dropout\\
$\mathcal{D}_p$ denotes a subset of a training dataset $\mathcal{D}$ that each LF contains the predicate $p$.
}
\label{algo:sup}
\end{algorithm}

==> meta-result_back.tex <==
%\begin{table}[ht]
%\centering
%{\small

\begin{table*}[ht]
\resizebox{0.9\textwidth}{!}{%
%\resizebox{0.9\textwidth}{!}{
\begin{tabular}[t]{@{} |l|ccc@{}||ccc@{}|}
\toprule
         & \Jobs & \Geo & \Atis & \Jobs & \Geo & \Atis\\ 
\midrule
\hline         
\seqseq (\pt)  & 11.27 $\pm$ 7.00  &  20.00 $\pm$ 5.12     &   17.23 $\pm$ 11.26  & 14.58 $\pm$ 8.63  &  33.01 $\pm$ 12.27     &   18.76 $\pm$ 10.09 \\
\seqseq (\os)  & 14.18 $\pm$ 7.84  &  11.38 $\pm$ 7.87     &   4.45 $\pm$ 3.74 & 30.46 $\pm$ 16.78  &  33.59 $\pm$ 10.11     &   10.17 $\pm$ 7.22 \\
\seqseq (\comb)  & 11.70 $\pm$ 8.86  &  7.64 $\pm$ 6.33     &   2.25 $\pm$ 4.96 & 21.49 $\pm$ 16.78  &  14.36 $\pm$ 9.38     &   7.91 $\pm$ 7.52 \\
%\hline
%\seqtree (\pt) & 9.82 $\pm$ 7.28  &  13.84 $\pm$ 8.91       &  7.96 $\pm$ 7.84  & 15.51 $\pm$ 6.72  &  28.45 $\pm$ 6.96       &  6.54 $\pm$ 3.07  \\
%\seqtree (\os) & 14.73 $\pm$ 10.57  &  8.72 $\pm$ 7.32       &  3.00 $\pm$ 2.19 & 19.44 $\pm$ 14.50  &  14.18 $\pm$ 5.53       &  5.24 $\pm$ 2.31  \\
%\seqtree (\comb) & 9.63 $\pm$ 9.07  &  13.17 $\pm$ 4.56       &  2.09 $\pm$ 1.64   & 18.50 $\pm$ 14.62  &  25.24 $\pm$ 7.33       &  8.13 $\pm$ 6.59  \\
\hline
\coarsefine (\pt) & 10.91 $\pm$ 4.94  & 24.07 $\pm$ 10.01       &  17.44 $\pm$ 9.82  & 13.83 $\pm$ 5.55  & 35.63 $\pm$ 8.97       &  21.08 $\pm$ 4.65 \\
\coarsefine (\os) & 6.73 $\pm$ 3.99  & 10.35 $\pm$ 11.48       &  5.26 $\pm$ 5.39 & 16.08 $\pm$ 11.22  & 28.55 $\pm$ 12.64      &  17.73 $\pm$ 9.48 \\
\coarsefine (\comb) & 9.28 $\pm$ 8.56  & 14.50 $\pm$ 11.44    &  0.42 $\pm$ 0.86 & 19.61 $\pm$ 8.39  & 28.93 $\pm$ 10.14       &  9.25 $\pm$ 6.16 \\
\hline
\irnet (\pt) & 16.00 $\pm$ 8.45  & 20.00 $\pm$ 10.86       &  17.12 $\pm$ 5.10  & 19.06 $\pm$ 7.63  & 35.05 $\pm$ 6.28       &  20.11 $\pm$ 8.44 \\
\irnet (\os) & 14.91 $\pm$ 7.78  & 18.78 $\pm$ 7.82       &  4.95 $\pm$ 5.35 & 30.84 $\pm$ 12.45  & 40.97 $\pm$ 10.20      &  18.05 $\pm$ 16.39 \\
\irnet (\comb) & 19.67 $\pm$ 12.07  & 21.90 $\pm$ 6.65    &  5.60 $\pm$ 4.97 & 28.22 $\pm$ 10.92  & 44.08 $\pm$ 2.73       &  15.73 $\pm$ 8.97 \\
\hline
\da     & 18.91 $\pm$ 11.83 & 9.67 $\pm$ 9.51     &  4.29 $\pm$ 5.55   & 21.31 $\pm$ 9.86 & 20.88 $\pm$ 21.56       &   17.18 $\pm$ 6.83  \\
\hline
\ptmaml     & 11.64 $\pm$ 4.65 & 9.76 $\pm$ 5.92     &  6.83 $\pm$ 5.33   & 17.76 $\pm$ 9.98 & 22.52 $\pm$ 12.47       &   12.28 $\pm$ 5.27  \\
\hline
Ours  & \textbf{27.09 $\pm$ 4.14}  & \textbf{27.49 $\pm$ 11.25}        & \textbf{19.27 $\pm$ 7.73}    & \textbf{32.5 $\pm$ 11.18} & \textbf{48.45 $\pm$ 5.71}        & \textbf{22.48 $\pm$ 3.82}    \\
\bottomrule

\end{tabular}%
}
\caption{Evaluation of learning results on three datasets. (Left) The one-shot results. (Right) The two-shot results.}

\label{table:meta}
\vspace{-3mm}
\end{table*}
%\end{subtable}

%\hspace{\fill}



%\begin{subtable}[ht]{.48\textwidth}


%\begin{tabular}[t]{@{} |l|ccc@{}|}
%\toprule
%         & \Jobs & \Geo & \Atis \\ 
%\midrule

%\hline         
%\seqseq (\pt) & 14.58 $\pm$ 8.63  &  33.01 $\pm$ 12.27     &   18.76 $\pm$ 10.09 \\
%\seqseq (\os) & 30.46 $\pm$ 16.78  &  33.59 $\pm$ 10.11     &   10.17 $\pm$ 7.22 \\
%\seqseq (\comb) & 21.49 $\pm$ 16.78  &  14.36 $\pm$ 9.38     &   7.91 $\pm$ 7.52 \\
%\hline
%\seqtree (\pt) & 15.51 $\pm$ 6.72  &  28.45 $\pm$ 6.96       &  6.54 $\pm$ 3.07  \\
%\seqtree (\os) & 19.44 $\pm$ 14.50  &  14.18 $\pm$ 5.53       &  5.24 $\pm$ 2.31  \\
%\seqtree (\comb) & 18.50 $\pm$ 14.62  &  25.24 $\pm$ 7.33       &  8.13 $\pm$ 6.59  \\
%\hline
%\coarsefine (\pt) & 13.83 $\pm$ 5.55  & 35.63 $\pm$ 8.97       &  21.08 $\pm$ 4.65 \\
%\coarsefine (\os) & 16.08 $\pm$ 11.22  & 28.55 $\pm$ 12.64      &  17.73 $\pm$ 9.48 \\
%\coarsefine (\comb) & 19.61 $\pm$ 8.39  & 28.93 $\pm$ 10.14       &  9.25 $\pm$ 6.16 \\
%\hline
%\ptmaml     & 16.07 $\pm$ 7.28 & 28.07 $\pm$ 13.03       &   16.15 $\pm$ 4.36  \\
%\hline
%Ours    & \textbf{32.5 $\pm$ 11.18} & \textbf{49.32 $\pm$ 3.18}        & \textbf{22.48 $\pm$ 3.82}    \\ \bottomrule
%\hline
%\end{tabular}
%\caption{Evaluation of two-shot learning results on three datasets}
%\end{subtable}


%\begin{table}[ht]
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{@{} c|ccc@{}}
%\toprule
%         & \Jobs & \Geo & \Atis \\ 
%\midrule

%\hline         
%\seqseq (\pt) & 14.58 $\pm$ 8.63  &  33.01 $\pm$ 12.27     &   18.76 $\pm$ 10.09 \\
%\seqseq (\os) & 30.46 $\pm$ 16.78  &  33.59 $\pm$ 10.11     &   10.17 $\pm$ 7.22 \\
%\seqseq (\comb) & 21.49 $\pm$ 16.78  &  14.36 $\pm$ 9.38     &   7.91 $\pm$ 7.52 \\
%\hline
%\seqtree (\pt) & 15.51 $\pm$ 6.72  &  28.45 $\pm$ 6.96       &  6.54 $\pm$ 3.07  \\
%\seqtree (\os) & 19.44 $\pm$ 14.50  &  14.18 $\pm$ 5.53       &  5.24 $\pm$ 2.31  \\
%\seqtree (\comb) & 18.50 $\pm$ 14.62  &  25.24 $\pm$ 7.33       &  8.13 $\pm$ 6.59  \\
%\hline
%\coarsefine (\pt) & 13.83 $\pm$ 5.55  & 35.63 $\pm$ 8.97       &  21.08 $\pm$ 4.65 \\
%\coarsefine (\os) & 16.08 $\pm$ 11.22  & 28.55 $\pm$ 12.64      &  17.73 $\pm$ 9.48 \\
%\coarsefine (\comb) & 19.61 $\pm$ 8.39  & 28.93 $\pm$ 10.14       &  9.25 $\pm$ 6.16 \\
%\hline
%\ptmaml     & 16.07 $\pm$ 7.28 & 28.07 $\pm$ 13.03       &   16.15 $\pm$ 4.36  \\
%\hline
%Ours    & \textbf{32.5 $\pm$ 11.18} & \textbf{49.32 $\pm$ 3.18}        & \textbf{22.48 $\pm$ 3.82}    \\ \bottomrule
%\hline
%\end{tabular}
%}
%\caption{Evaluation of two shot learning results on three datasets}
%\label{table:meta-two}
%\end{table}

==> sec1-intro-back.tex <==
We present a transition-based neural semantic parser, called prototypical semantic parser (\parser), that maps an utterance to an LF. Compared to prior neural semantic parsers, it extends a sequence-to-action neural parser~\cite{cheng2019executableParser} with Prototypical networks~\cite{snell2017prototypical} {in order to enable learning} the representations of new predicates. 
%
We design a novel attentional regularization method specific to facilitate finding alignments between NL constituents and predicates in the case of few training data. Furthermore, as a logical form in the few-shot setting consists of a mixture of known and new predicates, we propose a designated meta-learning method called \textit{predicate-dropout} to improve representation learning of such logical forms.   

Prior work~\cite{dong2018coarse2fine} found out that many LFs differ only in their mentioned atoms. In order to separate highly varying information from fixed structures, they create LF \textit{templates} by replacing each atom about entities or attribute values in LFs with slot variables and linking the corresponding atoms to the slot variables. Thus, an LF can also be viewed as a combination of an LF template and its slot values. The LF template from our example LF above takes the following form,
\begin{quote}
{\small
\begin{center}
    \begin{tabular}{c r}
    \label{example_template}
    \emph{(lambda \$0 e (exists \$1 (and ( ground\_transport \$1 )  }\\ 
     \emph{(to\_city \$1 \textbf{s0} )(from\_airport \$1 \textbf{s0}) ( =(ground\_fare \$1 ) \$0 ))))} % & (a)
    \end{tabular}
\end{center}
}
\end{quote}
\noindent where \emph{Vi} denotes the slot variables $i$ for the entity of the type state, ``6000'' and ``PhD'' are their corresponding slot values.

Formally, let $\vx = \{x_1, ... , x_n\}$ denote an NL utterance, and its LF is represented as a semantic tree $\vy = (V, E)$, where $V = \{v_1, ... , v_m\}$ \reza{should it be $\mathcal{V}$?} denotes the node set with $v_i \in \mathcal{V}$, and $E \subseteq \mathcal{V} \times \mathcal{V} $ is its edge set. As illustrate in~\todo , the node set $\mathcal{V} = \mathcal{V}_p \cup \mathcal{V}_v$ is further divided into a template predicate set $\mathcal{V}_p$ and a slot value set $\mathcal{V}_v$. A template predicate node represents a predicate symbol or a term, while a slot value node represents an atom mentioned in utterances. Thus, a semantic tree $\vy$ is composed of an abstract tree $\tau_{\vy}$ representing a template and a set of slot value nodes $V_{v,\vy}$ attaching to the abstract tree. \reza{should it be $\mathcal{V}_{v,\vy}$ ?}

Given utterances, we apply a neural transition system to generate templates, and a slot filling module to complete templates with slot values. To exploit shared structures of templates, we normalize the corresponding semantic trees into a compact form as a preprocessing step.
  
\includegraphics[width=\textwidth]{tree_unnorm.jpeg}
\subsection{Tree Normalization}
\label{sec:normalize_trees}
\begin{figure*}
\centering
\includegraphics[wide=\textwidth]{figures/}
\label{fig:normalized_tree_example}
\caption{An example of normalized abstract semantic tree}
\end{figure*}

\begin{table}[h!]
  \begin{center}
    \label{tab:act_len}
    \begin{tabular}{l|S|r|l}
      \textbf{Methods} & \textbf{Geo} & \textbf{Atis} & \textbf{Jobs}\\ 
      \hline
%      Seq2Seq & 15.5 & 25.5 & 15.1\\ % <--
%      Coarse2fine & 6.9 & 9.2 & -\\ % <--
      unnorm & 9.0 & 15.0 & 7.8\\ % <--
      norm & 4.8 & 6.8 & 3.7 \\ % <--
    \end{tabular}
    \label{table:num_actions_stat}
    \caption{The average number of parse actions per utterance.}
  \end{center}
\end{table}
Many LF templates in the existing corpora have shared subtrees in the corresponding abstract semantic trees. The reasons of treating such subtrees as single units are three folds. First, we avoid prediction errors that get parts of such subtrees wrong. Second, such subtrees often carry a consistent semantic meaning, such as \pre{(=(ground\_fare \$1) \$0)}. In contrast, the variable names in them are used for varying purposes across LFs, or some predicate symbols herein represents the same meaning as the subtrees. Third, it significantly reduces the size of semantic trees (Figure \ref{fig:normalized_tree_example}) and the number of parse actions per utterance. As shown in Table \ref{table:num_actions_stat}, the number of average actions taken for each utterance drops by almost 50\%. This number is also significantly less than the number of predictions per utterance for Seq2Seq and Coarse2fine. This normalization is a key difference to the prior works based on transition systems~\cite{chen2018seq2act, yin2018tranx}, which employ fine grained nodes such as variables and predicate symbols.
%\begin{center}
%    \emph{"answer(A, highest(A, (place(A), loc(A,B), state(B), const(B,stateid(V0))))))."}
%\end{center}
%for
%\begin{center}
%    \emph{Could you tell me what is the highest point in the state of Oregon?}
%\end{center}
%and
%\begin{center}
%    \emph{answer(A,(size(B,A),const(B,stateid(V0))))}
%\end{center}
%for
%\begin{center}
%    \emph{How big is alaska?}
%\end{center}
%
%Comparing these templates, it is easy to find out that there are shared clauses or structures. For example, \emph{const(B,stateid(V0))} and \emph{answer(A,B} are shared in all those templates. \emph{loc(A,B)} appears also in the first two templates. 
 %   All templates are formed in tree structures. It reflects the nature of Prolog that all programs can be formulated as a set of Horn clauses.
 
%We represent such a shared clause or structure as a single node because i) decomposing them into fine grained structures could lead to unnecessary parsing errors; ii) machine learning models cannot learn the substructures within those shared structures if a shared structure always acts as a single unit across the training dataset \reza{more intuition?}. 
%Theor work b concrete dto priefinition of DAGs depends on the grammar of the formal language.  

%Inspired by \cite{dong2018coarse2fine}, we decompose $P(y|x)$ into a two-stage generation process. 


%In~\cite{finegan2018improvingtexttosql}, they show that the SQL statements and logical forms can be reduced to a small number of such templates. In this example, the remaining task of semantic parsing is to fill the slot $VAR0$, which can be regarded as an NER and matching problem.

%An LF can be viewed as a tree with a node set $\mathcal{V}$ and an edge set $\mathcal{E}$. A tree $t$ with a node set $\mathcal{V}_t$ and an edge set $\mathcal{E}_t$ is called a \textit{subtree} if and only if $\mathcal{V}_t \subseteq \mathcal{V}$ and $\mathcal{E}_t \subseteq \mathcal{E}$. 
The identification of such shared structured is conducted by finding frequent subtrees. Given an LF database, the \textit{support} of a tree $t$ is the number of LFs that it occurs as a subtree. We call a tree \textit{frequent} if its support is greater and equal to a pre-specified minimal support.

We also observe that in an LF dataset, some frequent subtrees always have the same supertree. For example, \pre{ground\_fare \$1} is always the child of \textit{=( $\dots$, \$0 )} in the whole dataset. We call a subtree \textit{complete} w.r.t. a database if any of its supertrees in the dataset occur significantly more often than that subtree. 

%Another observation is that some tree nodes have fixed siblings. In order to check if two tree nodes sharing the same root are fixed siblings, we merge the two tree paths together. If the merged tree has the same support as that of the of the two trees, we call the two trees pass the fixed sibling test. In the same manner, we collapse tree nodes with fixed siblings, as well as their parent node into a single tree node to save unnecessary parse actions.

Thus, the normalization is conducted by collapsing a frequent complete abstract subtree into a tree node. We call a tree \textit{normalized} if all its frequent complete abstract subtrees are collapsed into the corresponding tree nodes. The pseudocode of the tree normalization algorithm is provided in Algorithm~\ref{algo:normalization}.
\begin{algorithm}
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\SetAlgoLined
\Input{A set of abstract trees $\mathcal{T}$, a minimal support $\tau$}
\Output{A set of normalized tress $\mathcal{N}$}
\For{$t$ in $\mathcal{T}$}{}
\label{algo:normalization}
\caption{Tree normalization.}
\end{algorithm}

\subsection{Transition System}
We apply the transition system~\cite{cheng2019executableParser} to perform a sequence of transition actions to generate the template of a normalized semantic tree. The transition system maintains partially-constructed outputs using a \textit{stack}. Parsing starts with an empty stack. At each step, a transition action is taken to update the parsing state and generate a tree node. The process repeats until the stack contains a complete tree.  

Formally, a parsing state is denoted by $c = (S,N,\Sigma)$, where $S$ is a stack, $N$ is the generated non-terminal symbols, and $\Sigma$ is the generated terminal symbols. In LF queries, a non-terminal symbol is the predicate symbol of a rule, while a terminal is an atom or a shared subtree. We take $c_0 = ([], \emptyset, \emptyset)$ as the initial state, and perform one of the following parse actions at each step.
\begin{itemize}
    \item \textbf{\gen{$y$}} creates a new terminal node $y \in \Sigma$ and pushes it on top of the stack.
    \item \textbf{\reduce{$r$}}. The reduce action identifies a rule $r$ taking the form $\text{head} :- \text{body}$. It attaches a new parent node to its children nodes on top of the stack. A parent node represents the head of a rule while its children nodes represent its rule body. The children nodes are first popped from the stack. Subsequently the parent node and the children nodes form a new subtree, which is pushed back to the stack.
\end{itemize}
Table \ref{table:example_transition} shows a transition sequence based on our running example. Similar to~\cite{cheng2019executableParser}, we require that the first action is \gen{$y$} during decoding. The parsing ends when the whole semantic tree (Figure \ref{}) is constructed. 
%\begin{figure}[h]
%\includegraphics[scale=0.5]{figures/parsing_graph.png}
%\caption{Example semantic tree.}
%\label{figure:example_semantic_tree}
%\end{figure}
\begin{small}
\begin{table*}[ht] % title of Table
\centering % used for centering table
\begin{tabular}{l c l} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
\textbf{t} & \textbf{Stack}& \textbf{Action} & % inserts table
%heading
\hline % inserts single horizontal line
t_1 & [] & \gen{(ground\_transport \$)}  \\
t_2 & [(ground\_transport \$)] & \gen{(to\_city \$ s0)}  \\
t_3 & [(ground\_transport \$), (to\_city \$ s0)] & \gen{(from\_airport \$ s1)}\\
t_4 & [(ground\_transport \$), (to\_city \$ s0), (from\_airport \$ s1)] & \gen{(= (ground\_fare \$) \$)}  \\
t_5 & [(ground\_transport \$), (to\_city \$ s0),&\\ & (from\_airport \$ s1), (= (ground\_fare \$) \$)] & \reduce{r}  \\
t_6 & [(and (ground\_transport \$) (to\_city \$ s0) } &\\ &(from\_airport \$ s1) (= (ground\_fare \$) \$))] & \reduce{r}\\%\reduce{h :- req\_deg(A,B), const(B,V1)}  \\
t_7 & [(exists \$ (and (ground\_transport \$) (to\_city \$ s0)} &\\ &(from\_airport \$ s1) (= (ground\_fare \$) \$)))] & \reduce{r}\\%\reduce{answer :- A, term+}\\
t_8 & [(lambda \$ e (exists \$ (and (ground\_transport \$) (to\_city \$ s0)} &\\ &(from\_airport \$ s1) (= (ground\_fare \$) \$))))] & \reduce{r}\\%\reduce{answer :- A, term+}\\
t_9 & [answer (lambda \$ e (exists \$ (and (ground\_transport \$) (to\_city \$ s0)} &\\ &(from\_airport \$ s1) (= (ground\_fare \$) \$))))] & \\ [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\caption{The transition sequence for LF template parsing "how much is the ground transportation between atlanta and downtown?".}
\label{table:example_transition} % is used to refer this table in the text
\end{table*}
\end{small}



\subsection{Neural Network Model}
We extend the neural semantic parser~\cite{cheng2019executableParser} with Prototypical Networks for coping with new predicates. Given a NL utterance $x$, we generate a sequence of actions $\mathbf{a} = a_1, ..., a_k$ to build a semantic tree $\tau_y$, which corresponds to a template. Then we complete the semantic tree $y$ by predicting the slot values $V_{y,v}$ and attach them as nodes to the abstract tree $\tau_y$. The learning goal is to estimate the probability $P(y, a |x)$.  
\begin{equation}
\label{eq:joint_prob_ya}
    P(y, \mathbf{a} |x) = P(y|\upsilon(\mathbf{a}), x) P(\mathbf{a}|x)
\end{equation}
where $P(\mathbf{a}|x)$ is the distribution for the transition system, 
%$P(\tau| a, x)$ implies an encoder to encode actions into a template representation (OPTIONAL), 
and $P(y|\upsilon(\mathbf{a}), x)$ denotes the distribution for slot filling. The function $\upsilon(\cdot)$ deterministically maps an action sequence $\mathbf{a}$ to an abstract tree $\tau_y$ by using rules.

The neural transition system consists of an encoder and decoder for estimating action probabilities.
\begin{equation}
    P(\mathbf{a} |x ) = \prod_{t = 1}^{|\mathbf{a}|} P(a_t | a_{<t},x)
\end{equation}
It modifies the decoder of an seq2seq model for coping with parsing states and action prediction. 

\paragraph{Encoder} We apply a bidirectional Long Short-term Memory (LSTM) network to map a squence of $n$ words into a sequence of contextual word representations $\{\mathbf{e}\}_{i=1}^n$. 

\paragraph{Decoder} The decoder applies a stack-LSTM \cite{dyer2015transition} to encode the stack of the transition system and action histories. A stack-LSTM extends unidirectional LSTM with a pointer pointing to the top element of the stack. Let $\mu_{t-1}$ and $\mathbf{h}^d_{t-1}$ denote the input and the hidden state of the LSTM at time $t$, the hidden state at $t$ is given by
\begin{equation}
    \mathbf{h}^d_t = \text{LSTM}(\mu_{t-1}, \mathbf{h}^d_{t-1})
\end{equation}
where $\mu_{t-1} = \begin{bmatrix}\mathbf{c}_{a_{t-1}}\\\mathbf{h}_{y_{t-1}} \end{bmatrix}$, which is a concatenation of the action embedding $\mathbf{c}_{a_{t-1}}$ and the subtree representation $\mathbf{h}_{y_{t-1}}$ predicted at time $t-1$.

If the action at time $t-1$ is \gen{$y_{t-1}$}, the decoder LSTM works the same as the vallina LSTM and reads the token $y_{t-1}$ as part of input. Otherwise if it is \reduce{r}, the action pops $k$ LSTM states corresponding to $k$ children nodes by moving the pointer to the state $\mathbf{h}^d_{t-k}$, and generate the representation of a new subtree by a linear transformation of the corresponding head and body representations of the rule.
\begin{equation}
    \mathbf{h}_{y_t} = \mathbf{M} \begin{bmatrix}\mathbf{c}_h\\ \frac{1}{k} \sum_{i = 1}^k \mathbf{h}^d_{t - i} \end{bmatrix}
\end{equation}
where $\mathbf{c}_h$ denotes the embedding of rule head $h$ and the rule body is represented by the mean of top $k$ hidden states of the LSTM. The LSTM creates a new branch of the LSTM at $t-k$ and reads the new subtree representation $\mathbf{h}_{y_t}$.
\begin{equation}
    \text{LSTM}(\begin{bmatrix}\mathbf{w}_{a_{t-1}}\\ \mathbf{h}_{y_t}\end{bmatrix}, \mathbf{h}^d_{t-k})
\end{equation}
If $m$ reduce actions are applied, the hidden states of stack-LSTM is not a sequence but have $m$ branches.

At each decoding step $t$, the top most hidden representation $\mathbf{h}_t$ is constructed by
\begin{equation}
    \mathbf{h}_t = \mathbf{W} \begin{bmatrix}
    \mathbf{h}_t^d\\
    \mathbf{h}_t^a
    \end{bmatrix}
\end{equation}
where $\mathbf{W}$ is a weight matrix and $\mathbf{h}^a_t$ is a attended representation created by soft attention\cite{luong2015effective}.
\begin{equation}
\label{eq:attented_rep}
    \mathbf{h}^a_t = \sum_{i=1}^n P(\mathbf{e}_i| \mathbf{h}^d_t)\mathbf{e}_i
\end{equation}
We apply dot product to compute the normalized attention scores $ P(\mathbf{e}_i| \mathbf{h}^d_t)$.

The probability of estimating an action is defined as:
\begin{equation}
\label{eq:action_prob}
P(a_t | \mathbf{h}_t) = \frac{\exp(\mathbf{c}_{a_t}^{\intercal} \mathbf{h}_t)}{\sum_{a' \in \mathcal{A}_t}\exp(\mathbf{c}_{a'}^{\intercal} \mathbf{h}_t)}
\end{equation}
where $\mathcal{A}_t$ denotes the set of applicable actions at time $t$, and $\mathbf{c}_{a}$ denotes the embedding of action $a$. As our definition of action has one-to-one relationship with the generated predicates, those action embeddings are regarded also as the representations of the corresponding predicates.

\paragraph{Slot Filling}
In few-shot learning, it is not realistic to expect that literals and atoms already exist in a lexicon. They may come either from a pre-defined lexicon or from utterances. Similar to \cite{yin2018tranx}, we employ a hybrid approach of generation and copying. In a normalized semantic tree, a tree node may involve more than one slot variables. Thus, given a node with slot variables, we aim to predict slot values of variable lengths.

We employ a LSTM based decoder that takes predicted slot values as input. The first hidden state of the LSTM is the representation of the corresponding tree node. At each time step $t$, we estimate a value $v$ by using a predictive distribution mixed with two types of slot value action \textit{gen} and \textit{copy}.

\begin{small}
\begin{align}\nonumber
    P(v | \mathbf{h}_t^v, x) =& P(v | \text{gen}, \mathbf{h}_t^v, x) (1 - P(\text{copy} | \mathbf{h}_t^v, x)) \\
    &+ P(v | \text{copy}, \mathbf{h}_t^v, x) P(\text{copy} | \mathbf{h}_t^v, x)
\end{align}
\end{small}
where $\mathbf{h}_t^v$ denotes the hidden state of the LSTM at time $t$.

The value generation probability $P(v | \text{gen}, \mathbf{h}_t^v, x)$ is estimated by $\text{softmax}(\mathbf{W}_v \mathbf{h}^v_t)$, where $\mathbf{W}_v$ is a embedding matrix for the pre-defined lexicon, which contains entity variable names and entities collected from training datasets. The probability $P(v | \text{copy}, \mathbf{h}_t^v, x)$ is estimated by the normalized attention scores $P(v |\mathbf{h}_t^v )$ that take the same form as Eq. \eqref{eq:attented_rep}, where $v$ denotes words from utterances. As we know the alignment between words and tree nodes with slot variables in training datasets, we maximize the probability of the correct alignment by optimizing the corresponding cross entropy during training. The remaining probability $P(\text{copy} | \mathbf{h}_t^v, x)$ is estimated by applying the Sigmoid function to the logit $\sigma(\mathbf{w}_c^\intercal \mathbf{h}_t^v)$.

%We start with adding a \textit{GEN($y_i$)} for each tree leaf node $y_i$. Then at each level, we recursively apply $REDUCE($r$)$ from left to right in order to generate the corresponding parent nodes. The process is repeated until all tree nodes are generated.

\subsection{Model Training}
We now introduce the designated meta-training method for training \parser in the few-shot settings. This method differs from conventional supervised training in three perspectives. First, it improves the representations of new predicates by using prototype vectors. Second, it applies a novel attention regularization to facilitate learning of alignments. Third, it involves a predicate-dropout method into the meta-learning procedure to simulate the testing scenarios.

One key idea of Prototypical networks is to construct prototype vectors as representations of new classification labels. The labels of new data points are determined by the labels of the most similar prototypes according a similarity measure. In light of this, we construct prototype vectors $\mathbf{c}_i$ for new predicates by taking the mean of the hidden representations at the corresponding time step $t$. More specifically, for all examples containing the action $a_t$ of a new predicate $p$ in the support set, its prototype vector is built by
\begin{equation}
    \mathbf{c}_p = \frac{1}{|M|}\sum_{\mathbf{h}_t \in M} \mathbf{h}_t
\end{equation}
where $M$ is the set of all hidden states for the prediction of the new predicate $p$.

It is difficult to obtain a good attention function when there are one or two examples per new predicate. We observe that the probability $P(a_j | x_i) = \frac{\text{count}(a_j, x_i)}{\text{count}(x_i)}$ and their character similarity  are often strong indicators of their alignment. In our work, we adopt $1 - dist(a_j, x_i)$ as the character similarity, where $dist(a_j, x_j)$ is normalized Levenshtein distance~\cite{levenshtein1966stringDistance}. Both measures are in the range $[0,1]$, thus we apply a sigmoid function $\sigma(\mathbf{w}^\intercal_p \mathbf{h}^d_t)$ $g(a_j, x_i) = \sigma(\cdot)P(a_j | x_i) + (1 - \sigma(\cdot)char\_sim(a_j, x_i)$ to combine them into a single score. The corresponding normalized attention scores is given by
\begin{equation}
    P'(x_i | a_k) = \frac{g(a_k, x_i)}{\sum_{j=1}^n g(a_k, x_j)}
\end{equation}
The attention scores $P(x_i | a_k)$ in Eq. \ref{eq:attented_rep} should be similar to $P'(x_i | a_k)$. Thus, we add a attention regularization term $\Omega = \sum_{ij} | P(x_i | a_j) - P'(x_i | a_j)|$ to our loss during training.

Our training procedure aims to simulate action sequence prediction in testing. In the testing of $k$ shot learning, we are provided with a support set, which contains $k$ sentence-LF pairs per new predicate. The final evaluation is on the test set, in which each LF contains at least one new predicate. However, there are no examples of new predicates in the training data.

Our preliminary experiments show that if there sufficient training data, it is better off training predicate embeddings $\mathbf{c}$ in a supervised way, while the model performs better when using prototype vectors for rarely occurred predicates. As we want to learn good representations in both cases, the loss is a combination of cross entropy $\mathcal{L}_s$ for known predicates and a meta loss $\mathcal{L}_m$ for templates of mixed predicates.
\begin{equation}
    \mathcal{L} = \mathcal{L}_s + \mathcal{L}_m + \lambda \Omega
\end{equation}
As $\mathcal{L}_s$ and $\mathcal{L}_m$ correspond to different subsets of data, we alternately use one batch for optimizing $\mathcal{L}_s$ and one batch for $\mathcal{L}_m$. The optimization on batches for $\mathcal{L}_s$ is the same as supervised learning. Given a batch for $\mathcal{L}_m$, we split the data into a meta-support set and a meta-query set. In order to simulate existence of new predicates, we randomly select a subset of actions as new, thus their representations $\mathbf{c}$ are prototype vectors constructed on the meta-support set. The remaining actions keep the representations learned supervisely from previous batches. The resulted action embedding matrix $\mathbf{C}$ is the combination of both.
\begin{equation}
\label{eq:action_embed_meta}
    \mathbf{C} = \mathbf{m}^\intercal \mathbf{C}_s + (1 - \mathbf{m}^\intercal) \mathbf{C}_p
\end{equation}
where $\intercal \mathbf{C}_s $ is the embedding matrix learned in a supervised way, and $\mathbf{C}_p$ is constructed by using prototype vectors on the meta-support set. The mask vector $\mathbf{m}$ is generated by randomly setting indices of some predicates to zero. We refer to this operation as \textit{predicate-dropout}. As in other meta-learning algorithms, the meta-loss is minimized on the meta-query set. Pseudocode of the algorithm for computing the meta-loss in one batch is provided in Algorithm \ref{algo:meta}.
\begin{algorithm}[H]
\label{algo:meta}
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\SetAlgoLined
\Input{Training set $\mathcal{D}$, a predicate set $\mathcal{P}$, a supervisely trained predicate embedding $\mathcal{C}_s$, number of shots $k$}
\Output{The loss $\mathcal{L}_m$ for a batch.}

Sample a subset $\mathcal{P}_i \sim \mathcal{P}$\\
$S$ := $\emptyset$\\
$Q$ := $\emptyset$\\
\For{p in $\mathcal{P}_i$}{
    Sample $S'$ of size $k$ from $\mathcal{D}_p$\\
    Sample $Q'$ of size $k$ from $\mathcal{D}_p$\\
    $S = S \cup S'$\\
    $Q = Q \cup Q'$\\
}
Build a prototype matrix $\mathcal{C}_p$ on $S$\\
Build a mask $\mathbf{m}$ using $\mathcal{P}_i$\\
Apply Eq. \eqref{eq:action_embed_meta} to compute $\mathbf{C}'$\\
Compute $\mathcal{L}_m$, the cross-entropy on $Q$ with $\mathbf{C}$
\caption{Predicate-Dropout\\
$\mathcal{D}_p$ denotes a subset of a training dataset $\mathcal{D}$ that each LF contains the predicate $p$.
}
\end{algorithm}
%\subsection{Training}
%\paragraph{Pretraining} Semantic parsing specific pretraining aims to construct high quality representations of text that are similar to prototypes of substructures in semantic DAGs. In another words, we want to automatically find constituent clusters during pretraining such that many cluster centroids can be directly used as prototypes of parse actions.
%\paragraph{Fine tuning with reinforcement learning}
%\paragraph{Cross template training with meta-learning}

%\paragraph{Soundness}

%\paragraph{Completeness}

% The query for the question \emph{"Are there convenience stores near Zum Wattkorn in Hamburg?"} is given as follows:

%\begin{center}
%    \begin{emph}
%    query( around( center( area( keyval('name','Hamburg')) , nwr( keyval('name','Zum Wattkorn') )) , search( nwr( keyval('shop','convenience') )) , maxdist(DIST\_INTOWN)) , qtype( least( topx(1) )))
%   \end{emph}
%\end{center}



==> sec3_fewshot_back.tex <==

\section{Semantic Parser}
\label{sec:template-general}
%We present a transition-based neural semantic parser, called prototypical semantic parser (\parser), that maps an utterance to an LF. From a modelling perspective, it extends a sequence-to-action neural parser~\cite{cheng2019executableParser} with Prototypical networks~\cite{snell2017prototypical} {in order to enable learning} the representations of new predicates \reza{how about the introduction of substructures (within templates) and the grammar to connect them together? i think we need to break Section 3 to two sections: (i) our new transition-based semantic parser, (ii) the fewshot learning of semantic parser (currently the contributions of few shot learning and new semantic papers are hard to teas apart and understand)}. 
%\reza{how about the introduction of substructures (within templates) and the grammar to connect them together? i think we need to break Section 3 to two sections: (i) our new transition-based semantic parser, (ii) the fewshot learning of semantic parser (currently the contributions of few shot learning and new semantic papers are hard to teas apart and understand)}
%
%In terms of the training process, we design a novel attentional regularization method specific to facilitate finding alignments between NL constituents and predicates in the case of few training data. Furthermore, as a logical form in the few shot setting consists of a mixture of known and new predicates, we propose a designated meta-learning method called \textit{predicate-dropout} to improve representation learning of such logical forms.   
In this section, we formally define the problem of semantic parsing in the few-shot setting, followed by presenting the transition system for template generation. Then we detail the model for both template generation and slot filling. 

%Prior work~\cite{dong2018coarse2fine} found out that many LFs differ only in their mentioned atoms, such as entities and attribute values. In order to separate highly varying information from fixed structures, they create LF \textit{templates} by replacing each atom in LFs with slot variables and linking the corresponding atoms to the slot variables. Thus, an LF can also be viewed as a combination of an LF template and its slot values (atoms). The LF template for our example LF in Introduction takes the following form
The same as the SOTA neural semantic parsers~\cite{dong2018coarse2fine}, our parser takes two steps to generate an LF: \textit{template generation} and \textit{slot filling}. An LF template is created by replacing the atom values in LFs with slot variables. The LF template of our example LF in Introduction is created by substituting i) a typed atom variable $v_e$ for the entity ``atlanta:ci''; ii) a shared variable name $v_a$ for all variables ``$\$0$`` and ``$\$1$``.

\vspace{-1mm}
{\small
\begin{center}
    \begin{tabular}{c r}
    \label{example_template}
    \emph{(lambda $v_a$ e (exists $v_a$ (and ( ground\_transport $v_a$ )  }\\ 
     \emph{(to\_city $v_a$ $v_e$ )(from\_airport $v_a$ $v_e$) ( =(ground\_fare $v_a$ ) $v_a$ ))))} % & (a)
    \end{tabular}
\end{center}
}
\noindent
Such LF templates are generated by our transition system, and the slot variables are replaced with the corresponding values by the slot filling module.

We found out LFs often contain idioms, which are frequent subtrees shared across LF templates. Thus we apply a \textit{template normalization} procedure in a similar manner as~\cite{iyer2019learningIdiomsSP} to preprocess all LF templates. It collapses idioms into single units such that all LF templates are converted into a compact form, see Appendix~\ref{app:normalize_trees} for details. 
%\noindent where $v_a$ and $v_e$ denote the slot variables for the attributes, ``$\$0$`` and ``$\$1$``, and the entity of the type location, ``atlanta:ci'', in the original LF.

%To exploit shared structures of templates, we uniquely propose a \textit{normalization} technique to convert the corresponding semantic trees into a compact form.
\subsection{Problem Statement}
%\begin{figure*}[t] 
%\centering
%\includegraphics[width=0.9\textwidth]{figures/semantic_both.pdf} 
%\vspace{-2mm}
%\caption{Trees from the the LF template ``\emph{(lambda $v_a$ e (exists $v_a$ (and ( ground\_transport $v_a$ )  }
%\emph{(to\_city $v_a$ $v_e$ )(from\_airport $v_a$ $v_e$) ( =(ground\_fare $v_a$ ) $v_a$ ))))} ''.
%(Left) The corresponding abstract semantic tree. (Right) The corresponding normalized tree. } %An example of normalized abstract semantic tree}
%\label{fig:normalized_tree_example}
%\vspace{-4mm}
%\end{figure*}

\begin{figure}

\begin{floatrow}
%
  \includegraphics[width=0.48\textwidth]{figures/semantic_tree.pdf}

\capbtabbox{
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l l} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
\textbf{t} & \textbf{Actions} \\ % inserts table
%heading
\hline % inserts single horizontal line
$t_1$ & \gen{(ground\_transport $v_a$)}  \\
$t_2$ &  \gen{(to\_city $v_a$ $v_e$)}  \\
$t_3$ &  \gen{(from\_airport $v_a$ $v_e$)}\\
$t_4$ &  \gen{(= (ground\_fare $v_a$) $v_a$)}  \\
$t_5$ &  \reduce{and :- NT NT NT NT}  \\
$t_6$ &  \reduce{exists :- $v_a$ NT}\\
$t_7$ &  \reduce{lambda :- $v_a$ e NT}\\
\hline %inserts single line
\end{tabular}
  }
  }{}
\end{floatrow}
\caption{Trees from the the LF template ``\emph{(lambda $v_a$ e (exists $v_a$ (and ( ground\_transport $v_a$ )  }
\emph{(to\_city $v_a$ $v_e$ )(from\_airport $v_a$ $v_e$) ( =(ground\_fare $v_a$ ) $v_a$ ))))} (Left) The corresponding abstract semantic tree. (Right) The action sequence, where "NT" denotes "non-terminal".}
\label{fig:tree_example}
\end{figure}


Formally, let $\vx = \{x_1, ... , x_n\}$ denote an NL utterance, and its LF is represented as a semantic tree $\vy = (\mathcal{V}, \mathcal{E})$, where $\mathcal{V} = \{v_1, ... , v_m\}$ denotes the node set with $v_i \in \mathcal{V}$, and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V} $ is its edge set. 
%As illustrated in Figure~\ref{fig:normalized_tree_example}, 
The node set $\mathcal{V} = \mathcal{V}_p \cup \mathcal{V}_v$ is further divided into a template predicate set $\mathcal{V}_p$ and a slot value set $\mathcal{V}_v$. A template predicate node represents a predicate symbol or a term, while a slot value node represents an atom mentioned in utterances. Thus, a semantic tree $\vy$ is composed of an abstract tree $\tau_{\vy}$ representing a template and a set of slot value nodes $\mathcal{V}_{v,\vy}$ attaching to the abstract tree.

In the few-shot setting, we are provided with a train set $\mathcal{D}_{train}$, a support set $\mathcal{D}_s$, and a test set $\mathcal{D}_{test}$. Each example in either of those sets is an utterance-LF pair $(\vx_i, \vy_i)$. The new predicates appear only in $\mathcal{D}_s$ and $\mathcal{D}_{test}$ but \textit{not} in $\mathcal{D}_{train}$. For $K$-shot learning, there are $K$ $(\vx_i, \vy_i)$ per each new predicate $p$ in $\mathcal{D}_s$. Each new predicate appears also in the test set. The goal is to maximize the accuracy of estimating LFs given utterances in $\mathcal{D}_{test}$ by using a parser trained on $\mathcal{D}_{train} \cup \mathcal{D}_{s}$. 
%Given utterances, we apply a neural transition system to generate templates, and a slot filling module to complete templates with slot values. To exploit shared structures of templates, we normalize the corresponding semantic trees into a compact form as a preprocessing step.
  
  
\subsection{Transition System}
We apply the transition system~\cite{cheng2019executableParser} to perform a sequence of transition actions to generate the template of a semantic tree. The transition system maintains partially-constructed outputs using a \textit{stack}. The parser starts with an empty stack. At each step, it performs one of the following transition actions to update the parsing state and generate a tree node. The process repeats until the stack contains a complete tree.  

%Formally, a parsing state is denoted by $S_t$, where $S_t$ is a stack storing a partial tree at time $t$. 
%The node set $\mathcal{V}$ of a partial tree is $N \cup \Sigma$, where $N$ is the set of generated non-terminal symbols, and $\Sigma$ is the generated terminal symbols. 
%In LFs, a non-terminal symbol is the predicate symbol of a rule, while a terminal is an atom or a idiom in the form of a subtree. 
% We take $S_0 = []$ as the initial state, and perform one of the following parse actions at each step.
\begin{itemize}
    \item \textbf{\gen{$y$}} creates a new terminal node $y$, which is an atom or a idiom in the form of a subtree, and pushes it on top of the stack.
    \item \textbf{\reduce{$r$}}. The reduce action identifies a rule $r$ taking the form, $\text{head} :- \text{body}$. The rules are automatically extracted from the data. It attaches a new parent node to its children nodes on top of the stack. A parent node represents the head of a rule while its children nodes represent its rule body. The children nodes are first popped from the stack. Subsequently the parent node and the children nodes form a new subtree to be pushed back to the stack.
\end{itemize}
An example transition sequence based on our running example is given in Figure \ref{fig:tree_example}.
 %shows a transition sequence based on our running example. 
%Similar to~\cite{cheng2019executableParser}, we require that the first action is \gen{$y$} during decoding. The parsing ends when the whole semantic tree is constructed.   

%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Tree Normalization}
%\label{sec:normalize_trees}
%\input{alg-tree-norm.tex}
%Many LF templates in the existing corpora have shared subtrees in the corresponding abstract semantic trees. The identification of such shared structured is conducted by finding subtrees which occurs more than $\tau$ times, namely the minimal \textit{support} of the frequent subtrees. The normalization is conducted by collapsing each frequent subtree into a tree node. %(Figure~\ref{fig:normalized_tree_example}). 
%The details of the tree normalization algorithm is provided in Algorithm \ref{algo:normalization}.
%Appendix~\ref{app:normalize_trees}.

%The reasons of treating such subtrees as single units are three folds. First, we avoid prediction errors that get parts of such subtrees wrong. Second, such subtrees often carry a consistent semantic meaning, such as \pre{(=(ground\_fare $v_a$) $v_a$)}. In contrast, the variable names in them are used for varying purposes across LFs, or some predicate symbols herein represents the same meaning as the subtrees. Third, as in Table~\ref{table:action_exp}, it significantly reduces the size of semantic trees and the number of parse actions per utterance. 
%As shown in Table~\ref{table:num_actions_stat}, 
%Given our study, the average length of actions taken for each utterance drops by almost 50\% after normalization. %This number is also significantly less than the number of predictions per utterance for Seq2Seq and Coarse2fine. 
%This normalization is a key difference to the prior works based on transition systems~\cite{chen2018seq2act, yin2018tranx}, which employ fine grained nodes such as variables and predicate symbols.

%\begin{table}[t]
%{\small
%  \begin{center}
%    \label{tab:act_len}
%    \begin{tabular}{l|ccc}
%    \toprule
%      Abstract Trees & \Geo & \Atis & \Jobs\\ 
%      \midrule
%      Seq2Seq & 15.5 & 25.5 & 15.1\\ % <--
%      Coarse2fine & 6.9 & 9.2 & -\\ % <--
%      Un-Normalized & 9.0 & 15.0 & 7.8\\ % <--
%      Normalized & 4.8 & 6.8 & 3.7 \\ % <--
%      \bottomrule
%    \end{tabular}
    
%    \caption{Average number of parse actions per utterance. }
%    \label{table:num_actions_stat}    
%  \end{center}
%  }
%   \vspace{-3mm}
%\end{table}

%\begin{table}[ht]

%\resizebox{\columnwidth}{!}{

%\begin{tabular}{l|l}
%\toprule
%Un-Normalized & Normalized\\ 
%  \midrule
%  \gen{$v_a$} & \gen{(= (ground\_fare $v_a$) $v_a$)}\\ % <--
%  \reduce{ground\_fare :- $v_a$} & ~ \\ % <--
%\gen{$v_a$} & ~ \\ % <--
%  \reduce{= :- (ground\_fare $v_a$) $v_a$} & ~ \\ % <--
%  \bottomrule
%\end{tabular}
%}
%\caption{The example transition action sequences to generate a semantic subtree, (= (ground\_fare $v_a$) $v_a$)))}
%\label{table:action_exp}


%   \vspace{-3mm}
%\end{table}

%\begin{table}[ht] % title of Table
%\centering % used for centering table
%\resizebox{\columnwidth}{!}{
%\begin{tabular}{l c l} % centered columns (4 columns)
%\hline\hline %inserts double horizontal lines
%\textbf{t} & \textbf{Un-Normalized}& \textbf{Normalized} \\ % inserts table
%heading
%\hline % inserts single horizontal line
%$t_1$ & \gen{$v_a$} & \gen{(ground\_transport $v_a$)}  \\
%$t_2$ & \gen{e} & \gen{(to\_city $v_a$ $v_e$)}  \\
%$t_3$ & \gen{$v_a$} & \gen{(from\_airport $v_a$ $v_e$)}\\
%$t_4$ & \gen{$v_a$} & \gen{(= (ground\_fare $v_a$) $v_a$)}  \\
%$t_5$ & \reduce{ground\_transport :- $v_a$} & \reduce{and :- NT NT NT NT}  \\
%$t_6$ & \gen{$v_a$} & \reduce{exists :- $v_a$ NT}\\
%$t_7$ & \gen{$v_e$} & \reduce{lambda :- $v_a$ e NT}\\
%$t_8$ & \reduce{to\_city :- $v_a$ $v_e$} & ~\\
%$t_6$ & \gen{$v_a$} & ~\\
%$t_7$ & \gen{$v_e$} & ~\\
%$t_8$ & \reduce{from\_airport :- $v_a$ $v_e$} & ~\\
%$t_9$ &  \gen{$v_a$} & ~\\ % <--
%$t_{10}$ &  \reduce{ground\_fare :- $v_a$} & ~ \\ % <--
%$t_{11}$ & \gen{$v_a$} & ~ \\ % <--
%$t_{12}$ &  \reduce{= :- NT $v_a$} & ~ \\ % <--
%$t_{13}$ &  \reduce{and :- NT NT NT NT} & ~ \\ % <--
%$t_{14}$ &  \reduce{exists :- $v_a$ NT} & ~ \\ % <--
%$t_{15}$ &  \reduce{lambda :- $v_a$ e NT} & ~ \\ % <--
%\hline %inserts single line
%\end{tabular}
%}
%\caption{The transition action sequence for the LF template parsing "how much is the ground transportation between atlanta and downtown?", where "NT" denotes "non-terminal".}
%\label{table:action_exp} % is used to refer this table in the text
% \vspace{-4mm}
%\end{table}
% parsing "how much is the ground transportation between atlanta and downtown?"

%\begin{center}
%    \emph{"answer(A, highest(A, (place(A), loc(A,B), state(B), const(B,stateid(V0))))))."}
%\end{center}
%for
%\begin{center}
%    \emph{Could you tell me what is the highest point in the state of Oregon?}
%\end{center}
%and
%\begin{center}
%    \emph{answer(A,(size(B,A),const(B,stateid(V0))))}
%\end{center}
%for
%\begin{center}
%    \emph{How big is alaska?}
%\end{center}
%
%Comparing these templates, it is easy to find out that there are shared clauses or structures. For example, \emph{const(B,stateid(V0))} and \emph{answer(A,B} are shared in all those templates. \emph{loc(A,B)} appears also in the first two templates. 
 %   All templates are formed in tree structures. It reflects the nature of Prolog that all programs can be formulated as a set of Horn clauses.
 
%We represent such a shared clause or structure as a single node because i) decomposing them into fine grained structures could lead to unnecessary parsing errors; ii) machine learning models cannot learn the substructures within those shared structures if a shared structure always acts as a single unit across the training dataset \reza{more intuition?}. 
%Theor work b concrete dto priefinition of DAGs depends on the grammar of the formal language.  

%Inspired by \cite{dong2018coarse2fine}, we decompose $P(y|x)$ into a two-stage generation process. 


%In~\cite{finegan2018improvingtexttosql}, they show that the SQL statements and logical forms can be reduced to a small number of such templates. In this example, the remaining task of semantic parsing is to fill the slot $VAR0$, which can be regarded as an NER and matching problem.

%An LF can be viewed as a tree with a node set $\mathcal{V}$ and an edge set $\mathcal{E}$. A tree $t$ with a node set $\mathcal{V}_t$ and an edge set $\mathcal{E}_t$ is called a \textit{subtree} if and only if $\mathcal{V}_t \subseteq \mathcal{V}$ and $\mathcal{E}_t \subseteq \mathcal{E}$.






%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\textwidth]{figures/semantic_tree.jpeg}
%    \label{fig:semantic_tree}
%    \caption{An example of semantic tree.}
%    \label{fig:my_label}
%\end{figure}

%\begin{figure}[h]
%\includegraphics[scale=0.5]{figures/parsing_graph.png}
%\caption{Example semantic tree.}
%\label{figure:example_semantic_tree}
%\end{figure}


\subsection{Parser Model}
\label{sec:nn_model}
%We present a transition-based neural semantic parser, called prototypical semantic parser (\parser), that maps an utterance to an LF. From a modelling perspective, it extends a sequence-to-action neural parser~\cite{cheng2019executableParser} with a Prototypical networks~\cite{snell2017prototypical}. In terms of the model training, as a logical form in the few shot setting consists of a mixture of known and new predicates, we propose a designated meta-learning method called \textit{predicate-dropout} to improve representation learning of such logical forms. Furthermore, we design a novel attentional regularization method specific to facilitate finding alignments between NL constituents and predicates in the case of few training data.

%we design a novel attentional regularization method specific to facilitate finding alignments between NL constituents and predicates in the case of few training data. Furthermore, as a logical form in the few shot setting consists of a mixture of known and new predicates, we propose a designated meta-learning method called \textit{predicate-dropout} to improve representation learning of such logical forms.   

%We extend the neural semantic parser~\cite{cheng2019executableParser} with Prototypical Networks for coping with new predicates.
\parser generates an LF in two steps: i) template generation, ii) slot filling.
\paragraph{Template generation} Given a NL utterance $x$, we generate a sequence of actions $\mathbf{a} = a_1, ..., a_k$ to build an abstract tree $\tau_{\vy}$, which corresponds to a template. Then we complete the semantic tree $\vy$ by predicting the slot values $\mathcal{V}_{v, \vy}$ and attach them as nodes to $\tau_{\vy}$. The learning goal is to estimate the probability $P(\vy, \va |\vx)$.
\begin{equation}
\label{eq:joint_prob_ya}
    P(\vy, \mathbf{a} |\vx) = P(\vy|\upsilon(\mathbf{a}), \vx) P(\mathbf{a}|\vx)
\end{equation}
where $P(\mathbf{a}|x)$ is the distribution for the transition system, 
%$P(\tau| a, x)$ implies an encoder to encode actions into a template representation (OPTIONAL), 
and $P(\vy|\upsilon(\mathbf{a}), \vx)$ denotes the distribution for slot filling. The function $\upsilon(\cdot)$ deterministically maps an action sequence $\mathbf{a}$ to an abstract tree $\tau_{\vy}$ by using deterministic rules.

The neural transition system consists of an encoder and a decoder for estimating action probabilities.
\begin{small}
\begin{equation}
    P(\mathbf{a} | \vx ) = \prod_{t = 1}^{|\mathbf{a}|} P(a_t | \va_{<t},\vx)
\end{equation}
\end{small}
It largely resembles~\cite{cheng2019executableParser} for coping with parsing states and action prediction. 

\textit{Encoder} We apply a bidirectional Long Short-term Memory (LSTM) network~\cite{gers1999LSTM} to map a squence of $n$ words into a sequence of contextual word representations $\{\mathbf{e}\}_{i=1}^n$. 

\textit{Decoder} The decoder applies a stack-LSTM \cite{dyer2015transition} to encode the stack of the transition system and action histories. A stack-LSTM is an unidirectional LSTM augmented with a pointer. The pointer points to the hidden state of the LSTM, which represents a particular state of the stack. It moves to a different hidden state to indicate a different state of the stack.%The stack-LSTM maps each stack status to a particular hidden state of the LSTM.

At time $t$, the LSTM $\mathbf{h}^d_t = \text{LSTM}(\mu_{t}, \mathbf{h}^d_{t-1})$ produces a hidden state $\mathbf{h}^d_{t}$ by taking $\mu_{t}$ as input, where $\mu_{t}$ is a concatenation of the embedding of the action $\mathbf{c}_{a_{t-1}}$ estimated at time $t-1$. The representation $\mathbf{h}_{y_{t-1}}$ of the partial tree at time $t-1$, which will be explained below.
%\begin{equation}
%    \mathbf{h}^d_t = \text{LSTM}(\mu_{t}, \mathbf{h}^d_{t-1})
%\end{equation}
One step of LSTM corresponds to \textit{push} $\mu_{t}$ into the stack, thus the pointer points to $\mathbf{h}^d_t$ after that.

At time $t-1$, if the action is \gen{$y_{t-1}$}, the partial tree representation $\mathbf{h}_{y_{t-1}}$ is the hidden state $\mathbf{h}^d_{t-1}$, because it was a \textit{push} operation at $t-1$. Otherwise if the action is \reduce{r}, it pops $k$ children nodes by moving the pointer to the state $\mathbf{h}^d_{t-k}$ and considers it as the state of $t-1$. The partial tree representation $\mathbf{h}_{y_{t-1}} = \mathbf{M} \begin{bmatrix}\mathbf{c}_{t-1}\\ \frac{1}{k} \sum_{i = 1}^k \mathbf{h}^d_{t - i} \end{bmatrix}$ is constructed by applying a linear transformation to the corresponding head and body representations of the rule, 
%\begin{equation}
%    \mathbf{h}_{y_{t-1}} = \mathbf{M} \begin{bmatrix}\mathbf{c}_{t-1}\\ \frac{1}{k} \sum_{i = 1}^k \mathbf{h}^d_{t - i} \end{bmatrix}
%\end{equation}
where the embedding of the rule head is denoted by $\mathbf{c}_{a_{t-1}}$ and the rule body is represented by the mean of top $k$ hidden states of the LSTM. After feeding both $\mathbf{h}_{y_{t-1}}$ and $\mathbf{c}_{a_{t-1}}$ to the LSTM, it creates a new branch at the state $\mathbf{h}^d_{t-k}$.

%Let $\mu_{t-1}$ and $\mathbf{h}^d_{t-1}$ denote the input and the hidden state of the LSTM at time $t$, the hidden state at $t$ is given by
%\begin{equation}
%    \mathbf{h}^d_t = \text{LSTM}(\mu_{t-1}, \mathbf{h}^d_{t-1})
%\end{equation}
%where $\mu_{t-1} = \begin{bmatrix}\mathbf{c}_{a_{t-1}}\\\mathbf{h}_{y_{t-1}} \end{bmatrix}$, which is a concatenation of the action embedding $\mathbf{c}_{a_{t-1}}$ and the subtree representation $\mathbf{h}_{y_{t-1}}$ predicted at time $t-1$.

%If the action at time $t-1$ is \gen{$y_{t-1}$}, the decoder LSTM works the same as the vallina LSTM and reads the token $y_{t-1}$ as part of input. Otherwise if it is \reduce{r}, the action pops $k$ LSTM states corresponding to $k$ children nodes by moving the pointer to the state $\mathbf{h}^d_{t-k}$, and generate the representation of a new subtree by a linear transformation of the corresponding head and body representations of the rule.
%\begin{equation}
%    \mathbf{h}_{y_t} = \mathbf{M} \begin{bmatrix}\mathbf{c}_h\\ \frac{1}{k} \sum_{i = 1}^k %\mathbf{h}^d_{t - i} \end{bmatrix}
%\end{equation}
%where $\mathbf{c}_h$ denotes the embedding of rule head $h$ and the rule body is represented by the mean of top $k$ hidden states of the LSTM. The LSTM creates a new branch of the LSTM at $t-k$ and reads the new subtree representation $\mathbf{h}_{y_t}$.
%\begin{equation}
%    \text{LSTM}(\begin{bmatrix}\mathbf{w}_{a_{t-1}}\\ \mathbf{h}_{y_t}\end{bmatrix}, %\mathbf{h}^d_{t-k})
%\end{equation}
%If $m$ reduce actions are applied, the hidden states of stack-LSTM is not a sequence but have $m$ branches.

As a common practice, $\mathbf{h}^d_{t}$ is concatenated with an attended representation $\mathbf{h}_t^a$ over encoder hidden states to yield $\mathbf{h}_t$, with
$
    \mathbf{h}_t = \mathbf{W} \begin{bmatrix}
    \mathbf{h}_t^d\\
    \mathbf{h}_t^a
    \end{bmatrix}
$, where $\mathbf{W}$ is a weight matrix. We apply dot product to compute the normalized attention scores $P(\mathbf{e}_i| \mathbf{h}^d_t)$ for $\mathbf{h}^a_t$~\cite{luong2015effective}. Given $\mathbf{h}_t$, the probability of an action is estimated by:
%\begin{equation}
%\label{eq:attented_rep}
%    \mathbf{h}^a_t = \sum_{i=1}^n P(\mathbf{e}_i| \mathbf{h}^d_t)\mathbf{e}_i
%\end{equation}
\begin{small}
\begin{equation}
\label{eq:action_prob}
P(a_t | \mathbf{h}_t) = \frac{\exp(\mathbf{c}_{a_t}^{\intercal} \mathbf{h}_t)}{\sum_{a' \in \mathcal{A}_t}\exp(\mathbf{c}_{a'}^{\intercal} \mathbf{h}_t)}
\end{equation}
\end{small}
where $\mathbf{c}_{a}$ denotes the embedding of action $a$, and $\mathcal{A}_t$ denotes the set of applicable actions at time $t$. 
%, we use the embedding of $y$ and the rule head of $r$ to represent the corresponding $\mathbf{c}_{a}$, respectively. 
The initialization of those embeddings will be explained in the following section.

\paragraph{Slot Filling}
% In few shot learning, it is not realistic to expect that literals and atoms already exist in a lexicon. They may come either from a pre-defined lexicon or from utterances. 
A tree node in a semantic tree may contain more than one slot variables due to template normalization. Since there are two types of slot variables, given a tree node with slot variables, we employ an LSTM-based decoder with the same architecture for each type of slot variables, respectively. The output of such a decoder is a value sequence of the same length as the number of slot variables of that type in the given tree node. 

For each tree node to predict, we set the initial state of the LSTM as the hidden state $\mathbf{h}_t$, which is used to generate the tree node (Eq. \eqref{eq:action_prob}). The first input of the LSTM is always fixed to \textit{$<$START$>$}. In the subsequential steps, an LSTM takes the slot value predicted at the previous time step as input. At each time step $t$, we estimate the probability of the slot value $P(v_t | \mathbf{h}_t, v_{1:t-1})$ by $\text{softmax}(\mathbf{W}_v \mathbf{h}^v_t)$, where $\mathbf{h}_t^v$ denotes the hidden state of the LSTM at time $t$ and $\mathbf{W}_v$ is a embedding matrix for that type of slot variables. The vocabulary of such a decoder is a pre-defined lexicon collected from training datasets. Since we know the number of each type of slots in a tree node, the prediction stops when $t$ reaches $T$.

%we employ two identical LSTM-based decoders on the top of the action prediction decoders to predict the attribute and entity values associated with each action $a$, respectively. The first hidden state of each LSTM is $\mathbf{h}^a_t$, the representation of the corresponding action. The first input of the LSTM is a starting token. Afterwards, each LSTM takes predicted slot values at last time step as input. At each time step $t$, we estimate the probability of the slot value $P(v_t | a, v_{1:t-1})$ by $\text{softmax}(\mathbf{W}_v \mathbf{h}^v_t)$, where $\mathbf{W}_v$ is a embedding matrix for the pre-defined lexicon, which contains either attribute or entity names collected from training datasets, and $\mathbf{h}_t^v$ denotes the hidden state of the LSTM at time $t$. Since the action $a$ records the number $T$ of each type of slots. The prediction stops when $t$ reaches $T$.

%by using a predictive distribution mixed with two types of slot value action \textit{gen} and \textit{copy}.

%\vspace{-2mm}
%\begin{small}
%\begin{align}\nonumber
%    P(v | \mathbf{h}_t^v, \vx) =& P(v | \text{gen}, \mathbf{h}_t^v, \vx) (1 - P(\text{copy} | \mathbf{h}_t^v, \vx)) \\
%    &+ P(v | \text{copy}, \mathbf{h}_t^v, \vx) P(\text{copy} | \mathbf{h}_t^v, \vx)
%\end{align}
%\end{small}
%where $\mathbf{h}_t^v$ denotes the hidden state of the LSTM at time $t$.

%The value generation probability $P(v | \text{gen}, \mathbf{h}_t^v, \vx)$ is estimated by $\text{softmax}(\mathbf{W}_v \mathbf{h}^v_t)$, where $\mathbf{W}_v$ is a embedding matrix for the pre-defined lexicon, which contains entity variable names and entities collected from training datasets. The probability $P(v | \text{copy}, \mathbf{h}_t^v, \vx)$ is estimated by the normalized attention scores $P(v |\mathbf{h}_t^v )$, where $v$ denotes words from utterances. As we know the alignment between words and tree nodes with slot variables in training datasets, we maximize the probability of the correct alignment by optimizing the corresponding cross entropy during training. The remaining probability $P(\text{copy} | \mathbf{h}_t^v, x)$ is estimated by applying the Sigmoid function to the logit $\sigma(\mathbf{w}_c^\intercal \mathbf{h}_t^v)$.

%We start with adding a \textit{GEN($y_i$)} for each tree leaf node $y_i$. Then at each level, we recursively apply $REDUCE($r$)$ from left to right in order to generate the corresponding parent nodes. The process is repeated until all tree nodes are generated.

\section{Few-Shot Model Training}
\input{alg-dropout.tex}
%\zhuang{I modified this part to a large degree, may someone pass this one to see whether it is fine? And now the order changed as well.}
The few-shot setting differs from the supervised setting by having a support set in testing in addition to train/test sets. The support set contains $k$ utterance-LF pairs per new predicate, while the training set contains only known predicates. To evaluate model performance on new predicates, the test set contains LFs with both known and new predicates. Given the support set, we can tell if a predicate is known or new by checking if it only exists in the train set. 

We take two steps to train our model: i) pre-training on the training set, ii) fine-tuning on the support set. Its predictive performance is measured on the test set. In the pre-training phase, we apply a training procedure involving \textit{predicate-dropout}, \textit{attention regularization}, and \textit{pre-training smoothing} to tackle the challenges due to data sparsity.

%The pre-training procedure of meta-learning should optimize the model for fast adaptability; hence the model could adapt to new task with few training examples. In light of this, the prototypical networks split each batch of training set into a meta-support set and a meta-test set. It applies the meta-support set to construct prototype vectors and minimize training errors on the meta-test set. The meta-support and meta-test sets are supposed to simulate the support and test sets that contain data points of new classes. 

In our experiments, we show that even for supervised parsers, it is better off pre-training them on the train set, followed by fine-tuning them on the support set. Meta-learning algorithms~\cite{snell2017prototypical,finn2017maml} suggest to simulate such splits during pre-training by splitting each batch into a meta-support set and a meta-test set. The models utilize the information on the meta-support set to minimize errors on the meta-test set. In this way, the meta-support and meta-test sets simulate the support and test sets that contain data points of new classes.

However, we cannot directly apply such a training procedure due to the following two reasons. First, each LF in the support and test sets is a mixture of both known predicates and new predicates. To simulate the support and test sets, the meta-support and meta-test sets in our setting should include both types of predicates as well. We cannot assume that there are only "new" predicates.
%In contrast, in standard prototypical network settings, each data point in a test set belongs to only new classes. 
Second, our preliminary experiments show that if there is sufficient training data, it is better off training action embeddings of known predicates $\mathbf{c}$ (Eq. \eqref{eq:action_prob}) in a supervised way, while the action embeddings initialized by a metric-based meta-learning algorithm~\cite{snell2017prototypical} perform better for rarely occurred new predicates in the fine-tuning step. Therefore, We cope with the differences between known and new predicates by a designated pre-training procedure and the targeted initialization methods in the fine-tuning step. 

%This method differs from conventional supervised training in three perspectives. First, it improves the representations of new predicates by initiallizing their embeddings by using prototype vectors. Second, it applies a novel attention regularization to facilitate learning of alignments. Third, it involves a predicate-dropout method into the meta-learning procedure to simulate the testing scenarios.
%Our training procedure aims to simulate action sequence prediction in testing. In the testing of $k$ shot learning, we are provided with a support set, which contains $k$ sentence-LF pairs per new predicate. The final evaluation is on the test set, in which each LF contains at least one new predicate. However, there are no examples of new predicates in the training data.
\paragraph{Pre-training with predicate-dropout} %Specifically, we propose a designated \textit{loss}, which is a combination of cross entropy $\mathcal{L}_s$, a meta loss $\mathcal{L}_m$ and an attention regularization term $\Omega$ with a coefficient term $\lambda$.
%The initialization methods aforementioned use prototype vectors for new predicates, while using random initialization for known predicates. We further improve the representations of both kinds of predicates in pre-training by using a designated \textit{loss}, which is a combination of cross entropy $\mathcal{L}_s$ for known predicates, a meta loss $\mathcal{L}_m$ for templates of mixed predicates and an attention regularization term $\Omega$ with a coefficient term $\lambda$.
The pre-training objective are two-folds: i) learn action embeddings for known predicates in a supervised way, ii) ensure that the model can learn good action embeddings of new predicates during fine-tuning.
 
Specifically, we propose a designated \textit{loss}, which is a combination of cross entropy $\mathcal{L}_s$, a meta loss $\mathcal{L}_m$ and an attention regularization term $\Omega$ with a coefficient term $\lambda$:
\begin{equation}
    \mathcal{L} = \mathcal{L}_s + \mathcal{L}_m + \lambda \Omega
\end{equation}

Starting with randomly initialized model parameters, we alternately use one batch for optimizing the supervised loss $\mathcal{L}_s$ and one batch for the meta-loss $\mathcal{L}_m$. We adopt cross-entropy for $\mathcal{L}_s$. In a batch for $\mathcal{L}_m$, we split the data into a meta-support set and a meta-test set. The meta-support set is used to construct the action embeddings and $\mathcal{L}_m$ would be minimized over the meta-test set. In order to simulate existence of new predicates, we randomly select a subset of predicates as new, thus their action embeddings $\mathbf{c}$ in Eq. \eqref{eq:action_prob} are replaced by prototype vectors as in prototypical networks~\cite{snell2017prototypical}. 
%We construct prototype vectors $\mathbf{c}_{a_t}$ of the actions $a_t$ associated with new predicates from the support set by taking the mean of the hidden representations at the corresponding time step $t$, because those hidden representations are supposed to be similar to their action embeddings. 
Formally, a prototype vector is built by taking the mean of a set of hidden states $\mathbf{h}_t$ obtained from the decoder when forwarding the parser model on the meta-support set.
\begin{equation}
    \mathbf{c}_{a_t} = \frac{1}{|M|}\sum_{\mathbf{h}_t \in M} \mathbf{h}_t
    \label{eq:action_embed_proto}
\end{equation}
where $M$ is the set of all hidden states for the prediction of the action $a_t$.
The action embeddings for the remaining predicates are learned from previous batches. The resulted action embedding matrix $\mathbf{C}$ is the combination of both.
%As $\mathcal{L}_s$ and $\mathcal{L}_m$ correspond to different subsets of data, we alternately use one batch for optimizing $\mathcal{L}_s$ and one batch for $\mathcal{L}_m$. The optimization on batches for $\mathcal{L}_s$ is the same as supervised learning. Given a batch for $\mathcal{L}_m$, we split the data into a meta-support set and a meta-test set. In order to simulate existence of new predicates, we randomly select a subset of predicates as new, thus their representations $\mathbf{c}$ are prototype vectors constructed on the meta-support set. The remaining predicates keep the representations learned from previous supervised batches. The resulted predicate embedding matrix $\mathbf{C}$ is the combination of both.
\begin{equation}
\label{eq:action_embed_meta}
    \mathbf{C} = \mathbf{m}^\intercal \mathbf{C}_s + (1 - \mathbf{m}^\intercal) \mathbf{C}_m
\end{equation}
where $\mathbf{C}_s $ is the embedding matrix learned in a supervised way, and $\mathbf{C}_m$ is constructed by using prototype vectors on the meta-support set. The mask vector $\mathbf{m}$ is generated by randomly setting indices of some predicates to zero. We refer to this operation as \textit{predicate-dropout}. The meta-training algorithm is summarised in Algorithm \ref{algo:sup}.

\paragraph{Fine-tuning} In the fine-tuning step, we initialize action embeddings for known predicates with the action embeddings learned during pre-training, while using prototype vectors by applying Eq. \eqref{eq:action_embed_proto} over the support set to initialize the ones for new predicates. After initialization, the whole model parameters are fine-tuned on the support set by using a cross entropy loss with attention regularization, $\mathcal{L} = \mathcal{L}_s + \lambda \Omega$. The prediction of templates is carried out by beam search of optimal action sequences.

\paragraph{Attention Regularization} We address the poorly learned attention scores $P(\mathbf{e}_i| \mathbf{h}^d_t)$ of infrequent actions by introducing a novel attention regularization. We observe that the probability $P(a_j | x_i) = \frac{\text{count}(a_j, x_i)}{\text{count}(x_i)}$ and their character similarity are often strong indicators of their alignment. In our work, we adopt $1 - dist(a_j, x_i)$ as the character similarity, where $dist(a_j, x_j)$ is normalized Levenshtein distance~\cite{levenshtein1966stringDistance}. Both measures are in the range $[0,1]$, thus we apply $g(a_j, x_i) = \sigma(\cdot)P(a_j | x_i) + (1 - \sigma(\cdot)char\_sim(a_j, x_i)$ to compute alignment scores, where the sigmoid function $\sigma(\mathbf{w}^\intercal_p \mathbf{h}^d_t)$ combines two measures into a single score. The corresponding normalized attention scores is given by
\begin{equation}
    P'(x_i | a_k) = \frac{g(a_k, x_i)}{\sum_{j=1}^n g(a_k, x_j)}
\end{equation}
The attention scores $P(x_i | a_k)$ should be similar to $P'(x_i | a_k)$. Thus, we define the regularization term as $\Omega = \sum_{ij} | P(x_i | a_j) - P'(x_i | a_j)|$ during training.

%of the algorithm for computing the meta-loss in one batch is provided in Algorithm \ref{algo:meta}.
\paragraph{Pre-training smoothing} Due to the new predicates, the number of candidate actions during the prediction of fine-tuning and testing is larger than the one during pre-training. That leads to distribution discrepancy between pre-training and testing. To minimize the differences, we assume a prior knowledge on the number of actions for new predicates by adding a constant $k$ to the denominator of Eq. \eqref{eq:action_prob} when estimating the action probability $P(a_t | \mathbf{h}_t)$ during pre-training. 
\begin{equation}
\label{eq:smooth}
P(a_t | \mathbf{h}_t) = \frac{\exp(\mathbf{c}_{a_t}^{\intercal} \mathbf{h}_t)}{\sum_{a' \in \mathcal{A}_t}\exp(\mathbf{c}_{a'}^{\intercal} \mathbf{h}_t) + k}
\end{equation}
We do not consider this smoothing technique during fine-tuning and testing.  
Despite its simplicity, the experimental results show a significant performance gain on benchmark datasets.

%\subsection{Training}
%\paragraph{Pretraining} Semantic parsing specific pretraining aims to construct high quality representations of text that are similar to prototypes of substructures in semantic DAGs. In another words, we want to automatically find constituent clusters during pretraining such that many cluster centroids can be directly used as prototypes of parse actions.
%\paragraph{Fine tuning with reinforcement learning}
%\paragraph{Cross template training with meta-learning}

%\paragraph{Soundness}

%\paragraph{Completeness}

% The query for the question \emph{"Are there convenience stores near Zum Wattkorn in Hamburg?"} is given as follows:

%\begin{center}
%    \begin{emph}
%    query( around( center( area( keyval('name','Hamburg')) , nwr( keyval('name','Zum Wattkorn') )) , search( nwr( keyval('shop','convenience') )) , maxdist(DIST\_INTOWN)) , qtype( least( topx(1) )))
%   \end{emph}
%\end{center}



==> tab-training.tex <==
\begin{table}[ht]
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{|@{} l|ccc@{}||ccc@{}|}
\toprule
         & \Jobs & \Geo & \Atis  & \Jobs & \Geo & \Atis \\ 
\midrule
ep & 120 & 20 & 30 & 60 & 80 & 40 \\

lr & 0.0005 & 0.0005  & 0.0005 & 0.0005 & 0.001 & 0.001 \\
att-reg  & 0.001 & 0.1 & 1 & 0.00001 & 0.1 & 1 \\
\bottomrule
\end{tabular}%
}
\caption{Hyperparameters of fine-tuning. (Left) The one-shot settings. (Right) The two-shot settings.}
\label{table:train}
\end{table}
\FloatBarrier

==> tab-valid.tex <==
\begin{table}[ht]
{\small
\begin{tabular}{|@{} l|ccc@{}||ccc@{}|}
\toprule
         & \Jobs & \Geo & \Atis\\ 
\midrule
one-shot & 46.36 & 17.54 & 22.77  \\

two-shot & 31.78 & 43.69  & 35.57 \\
\bottomrule
\end{tabular}%
}
\caption{Evaluation results of the one-shot and two-shot settings on the validation sets.}
\label{table:valid}
 %\vspace{-3mm}
\end{table}
